A General Retraining Framework for Scalable Adversarial Classification

Traditional classification algorithms assume that training and test data come from similar distributions. This assumption is violated in adversarial settings, where malicious actors modify instances to evade detection. A number of custom methods have been developed for both adversarial evasion attacks and robust learning. We propose the first systematic and general-purpose retraining framework which can: a) boost robustness of an \emph{arbitrary} learning algorithm, in the face of b) a broader class of adversarial models than any prior methods. We show that, under natural conditions, the retraining framework minimizes an upper bound on optimal adversarial risk, and show how to extend this result to account for approximations of evasion attacks. Extensive experimental evaluation demonstrates that our retraining methods are nearly indistinguishable from state-of-the-art algorithms for optimizing adversarial risk, but are more general and far more scalable. The experiments also confirm that without retraining, our adversarial framework dramatically reduces the effectiveness of learning. In contrast, retraining significantly boosts robustness to evasion attacks without significantly compromising overall accuracy.

==> sections_paper/attacks__bo_li_s_conflicted_copy_2016-02-11_.tex <==
\section{Modeling Attackers}

\subsection{Evasion Attack as Optimization}
\label{s:game}

In prior literature, evasion attacks have almost universally been
modeled as optimization problems in which attackers balance the
objective of evading the classifier (by changing the label from $+1$
to $-1$) and the cost of such
evasion~\cite{lowd2005adversarial,li2014feature}.
Our approach is in the same spirit, but is formally somewhat distinct.
In particular, we assume that the adversary has the following
two competing objectives: 1) appear as benign as possible to the
classifier, and 2) minimize modification cost.
Moreover, we assume that the attacker obtains no value from a
modification to the original feature vector if the result is still
classified as malicious.
To formalize, consider an attacker who in the original training data
uses a feature vector $x_i$ ($i \in I_{bad})$).
The adversary $i$ is solving the following optimization problem:
\begin{equation}
\label{eq:attack}
\min_{x \in X} \min\{0,f(x)\} + c(x,x_i).
\end{equation}
As is typical in related literature, we assume that $c(x,x_i) \ge 0$,
$c(x,x_i) = 0$ iff $x = x_i$, and $c$ is strictly increasing
in $\|x - x_i\|_2$ and strictly convex in $x$.
Because Problem~\ref{eq:attack} is non-convex, we instead minimize an upper bound:
\begin{equation}
\label{eq:attacker_q}
\min \limits_{x} Q(x) \equiv f(x) + c(x,x_i).
\end{equation}
In addition, if $f(x_i) < 0$, we return $x_i$ before solving Problem~\ref{eq:attacker_q}.
If Problem~\ref{eq:attacker_q} returns an optimal solution $x^*$ with
$f(x^*) \ge 0$, we return $x_i$; otherwise, return $x^*$.
Problem~\ref{eq:attacker_q} has two advantages.
First, if $f(x)$ is convex and $x$ real-valued, this is a (strictly) convex
optimization problem, has a unique solution, and we can solve it in polynomial time.
An important special case is when $f(x) = w^Tx$.
The second one we formalize in the following lemma.
\begin{lemma}
\label{L:bound}
Suppose $x^*$ is the optimal solution to Problem~\ref{eq:attack}, $x_i$ is
suboptimal, and $f(x^*) < 0$. 
Let $\bar{x}$ be the optimal solution to
Problem~\ref{eq:attacker_q}.
Then $f(\bar{x}) + c(\bar{x},x_i) = f(x^*) + c(x^*,x_i)$, and
$f(\bar{x}) < 0$.
\end{lemma}
\begin{proof}
If $f(x^*) < 0$, then $\min\{0,f(x^*)\} + c(x^*,x_i) = f(x^*) +
c(x^*,x_i)$.
By optimality of $\bar{x}$, $f(\bar{x}) + c(\bar{x},x_i) \le f(x^*) +
c(x^*,x_i)$.
Since $x_i$ is suboptimal in Problem~\ref{eq:attack} and $c$ strictly
positive in all other cases, $f(x^*) +
c(x^*,x_i) < 0$.
By optimality of $x^*$, $f(x^*) + c(x^*,x_i) \le \min\{0,f(\bar{x})\}
+ c(\bar{x},x_i) \le f(\bar{x}) + c(\bar{x}, x_i)$, which implies that
$f(\bar{x}) + c(\bar{x},x_i) = f(x^*) + c(x^*,x_i)$.
Consequently, $f(\bar{x}) + c(\bar{x},x_i) < 0$, and, therefore,
$f(\bar{x}) < 0$.
\end{proof}
The following corollary then follows by uniqueness of optimal
solutions for strictly convex objective functions over a real vector space.
\begin{corollary}
\label{C:convex}
If $f(x)$ is convex and $x$ continuous, $x^*$ is the optimal solution to
Problem~\ref{eq:attack}, $\bar{x}$ is the optimal solution to
Problem~\ref{eq:attacker_q}, and $f(x^*) < 0$, then $\bar{x} = x^*$.
\end{corollary}
A direct consequence of this corollary is that when we use
Problem~\ref{eq:attacker_q} to approximate Problem~\ref{eq:attack} and
this approximation is convex, we always return either the optimal
evasion, or $x_i$ if no cost-effective evasion is possible.
An oracle $\mathcal{O}$ constructed on this basis will therefore
return a unique solution, and supports the theoretical
characterization of \emph{RAD} above.

The results above are encouraging, but many learning problems do not
feature a convex $f(x)$, or a continuous feature space.
Next, we consider several general algorithms for adversarial evasion.

%In order to evade detections, the attacker aims to modify the original malicious instance $x^A$ to generate $x'$, which can be classified as benign, using limited budget. In general, the adversary needs to solve the optimization as below.

%\begin{align}
%\label{eq:attacker_model}
%x' = &\arg\min \limits_{x} f(x) \\
%s.t. \qquad &c(x', x^A) \leq d_{max}
%\end{align}

%Here $f(x)$ is the probability function learned by the classifier and $d_{max}$ is the maximum cost (budget) that the attacker is restricted to.  
%With binary features, Lowd and Meek have proposed a 2-approximate algorithm to generate such optimal evasion attack instances \cite{lowd2005adversarial}. They demonstrated that to generate the benign instance $x'$, the attacker at most need to pay twice of the ideal optimal cost. But this only applies to linear classifier and the budget of attacker cannot be bounded by certain values, which is often the case in practical. 

%Therefore we incorporate the cost of attackers into their objective, and form the adversary's objective as the following optimization problem.
%\begin{equation}
%\label{eq:attacker_g}
%\min \limits_{x'} H(x') := g(x') +\exp \left({\lambda \sqrt{\sum \limits_{i = 1}^n{ (x^A}_i -{x'}_i)^2 +1}} \right),
%\end{equation}
%where $g(x)$ is the sign function for the probability model $f(x)$.
%Therefore, we form the relaxation model for the original problem as below.
%\begin{equation}
%\label{eq:attacker_q}
%\min \limits_{x'} Q(x') := f(x') +\exp \left({\lambda \sqrt{\sum \limits_{i = 1}^n{ (x^A}_i -{x'}_i)^2 +1}} \right)
%\end{equation}

%Here $Q(x')$ indicates the adversarial minimization goal by modifying the adversarial instance $x^A$ into $x'$. 
%It is obvious that if the the optimal solution $x^*$ for the relaxed problem~\ref{eq:attacker_q} is feasible for the original problem, then it is also optimal for the original problem~\ref{eq:attacker_g}.
%We will discuss how to solve this adversarial optimization problem later in for different models in different cases later.

%We form the interaction between the learner and attacker as a Stackelberg game. Within the game, first the learner uses training data to choose a classifier $g(x)$, which can be viewed as a sign function of the probabilistic modeling function $f(x)$.
%Then each adversary applies a query-based algorithm to (approximately) solve the optimization problem~\ref{eq:attacker_model} for their malicious instances $x^A$ and generate their ``optimal" evasion instances to evade the classifier.
%Finally, the learner's loss is measured using a new dataset in which every malicious $x \in X$ is replaced with a corresponding $x'$ computed by optimizing the relaxed adversarial objective~\ref{eq:attacker_q}. 

%Within the game, given the knowledge (prediction) about the attacker behavior, the learner would optimize a more robust learning system by generating the adversarial strategies and include them for during training to enhance the model.
%The mixed integer programming approach, which can guarantee to find the optimal adversarial strategies $x^*$, was proposed in \cite{li2014feature}. However, this approach is not scalable for either the number of instances or feature dimensions.
%Therefore, we will discuss the coordinate greedy algorithm which is highly scalable, and the corresponding loss guarantee.

\subsection{Coordinate Greedy}
\label{s:coor}

%\subsubsection{Binary Feature Space}
We propose a very general local search framework,
\emph{CoordinateGreedy (CG)} (Algorithm~\ref{alg:coordinate} for approximating
optimal attacker evasion.
%To optimize the adversarial objective, we simulate the attacker's
%instances by coordinate descent algorithm\ref{alg:coordinate}.
\begin{algorithm}[thb]
\caption{CoordinateGreedy: $\mathcal{O}(\beta,x)$}
\label{alg:coordinate}
\begin{algorithmic}[1]
\STATE \textbf{Input}: {Parameter vector $\beta$, malicious instance $x$}
 \STATE {Set $k \leftarrow 0$ and let $x^0 \leftarrow x$}
 % \WHILE {$k < B$ and $f(x^k) \geq \delta$ }
 \REPEAT 
 % {$|f(x^A)-f(x^k)| \leq \delta$}
 \STATE{Randomly choose index $i_k \in \{1, 2, ..., n\}$ }
 \STATE{$x^{k+1} \leftarrow $GreedyImprove($i_k$)}
 %\STATE{$x^{k+1} \leftarrow x^k - \tau_k {[\triangledown Q(x^k)]}_{i_k} e_{i_k}$}
 \STATE {$k \leftarrow k+1$}
 % \UNTIL {$|Q(x^{k})-Q(x^{k-1})| \leq \epsilon$ or $f(x^k) \leq \delta$}
 %\UNTIL {$\frac{\ln Q(x^{k})} {\ln Q(x^{k-1})} \leq \epsilon$ or
 %$f(x^k) \leq \delta$}
 \UNTIL{$\frac{\ln Q(x^{k})} {\ln Q(x^{k-1})} \leq \epsilon$}
 % \ENDWHILE
% \STATE {Project $x^{k}$ to the feature space $x' \in X$}
\IF{$f(x^k) \ge 0$}
 \STATE $x^k \leftarrow x$
\ENDIF
 \STATE \textbf{Output}: {Adversarially optimal instance $x^k$.}
\end{algorithmic}
\end{algorithm}
The high-level idea is to iteratively choose a feature, and greedily
update this feature to incrementally improve the attacker's utility
(as defined by Problem~\ref{eq:attacker_q}).
In general, this algorithm will only converge to a locally optimal
solution.
We therefore propose a version with random restarts: run \emph{CG}
from $L$ random starting points in feature space, in addition to
starting from the initial malicious instance $x$.
As long as a global optimum has a basin of attraction with positive
Lebesgue measure, or the feature space is finite, this process will asymptotically converge to a
globally optimal solution as we increase the number of random
restarts.
%In practice, we would limit the number of these to be relatively
%small.
Thus, as we increase the number of random restarts, we expect to increase
the frequency that we actual return the global optimum.
Let $p_L$ denote the probability that the oracle based on coordinate
greedy with $L$ random restarts returns a suboptimal solution to Problem~\ref{eq:attacker_q}.
The next result generalizes the bound on \emph{RAD} to allow for this,
restricting however that the loss function which we bound from above
is the $0/1$ loss.
Let $\mathcal{L}_{A,01}^*(\mathcal{O})$ correspond to the total
adversarial loss in Equation~\ref{E:advloss}, where the loss function
$l(g_\beta(x),y)$ is the $0/1$ loss.
Suppose that $\mathcal{O}_L$ uses coordinate greedy with $L$ random restarts.
\begin{proposition}
\label{prop:defender_loss}
Let $B = |I_{bad}|$.
$\mathcal{L}_{A,01}^*(\mathcal{O}) \le \mathcal{L}^R_N(\beta,
\mathcal{O}_L) + \delta(p)$ with probability at least $1-p$, where 
% $\delta(p) = (p_L +
% (-\frac{1}{2B} \log p)^{1/2})$, 
$\delta(p) = B \cdot p_L + \frac{\sqrt{\log^2 p-8 B p_l \log p}-\log p}{2}$,
and $\mathcal{L}^R_N(\beta,
\mathcal{O}_L)$ uses any loss function $l(g_\beta(x),y)$ which is an upper bound on
the $0/1$ loss.
%The upper bound of defender's loss in adversarial environments is 
% $L_D \leq \sum \limits_{y_i = -1} l(-w^T x_i) + \sum \limits_{y_i = +1} \max \limits_{{x_i}' \in {x_i}^*} l(w^T {x_i}') + \lambda ||w||_p $.
%${L_D}^A \leq \sum \limits_{x_i \in X \cup R} l_\beta( x_i) + \alpha ||\beta||_p + t \cdot {P}_A$ when $f(x)$ is not convex, where $X$ is the original training set and $R$ represents the total added instances. $t$ denotes the number of malicious instances in $X$ ($t = |X_A|$), and $P_A$ is the probability that the best response $x^*$ would evade the classifier. 
\end{proposition}
\begin{proof}
%From Proposition~\ref{prop:defender_loss}, we have ${L_D}^A \leq \sum \limits_{x_i \in X \cup R} l_\beta( x_i) + \alpha ||\beta||_p$ if the adversary best response $x^* \in R$. However, if the adversary best response $x^*$ is not found and it can evade the classifier $g(x^*) =-1$, the loss of learner would increase with 1 for the 0-1 loss. Therefore, if the probability of the adversary best response $x^*$ evading classifier is $P_A$, 
%${L_D}^A \leq \sum \limits_{x_i \in X \cup R} l_\beta( x_i) + \alpha
%||\beta||_p + t \cdot {P}_A$.
Let $\bar{\beta} \in \arg\min_{\beta}  \mathcal{L}^R_N(\beta,
\mathcal{O}_L)$.
Consequently, for any $\beta$,
% (omitting regularization terms, since
% they are identical throughtout),
\begin{align*}
\mathcal{L}_{A,01}^*(\mathcal{O}_L) &= \min_\beta \mathcal{L}_{A,01}(\beta;
\mathcal{O}_L) \\
&\le \sum_{i: y_i = -1} l_{01}(g_{\bar{\beta}}(x_i),-1) +\\
&\quad\quad\quad\quad \sum_{i:y_i = +1}
l_{01}(g_{\bar{\beta}} (\mathcal{O}(\bar{\beta},x_i)),+1) + \alpha ||\bar{\beta}||_p^p.
\end{align*}
Now,
\begin{align*}
\sum_{i:y_i = +1} &l_{01}(g_{\bar{\beta}}
(\mathcal{O}(\bar{\beta},x_i)),+1) \le \\
&\sum_{i:y_i = +1} l_{01}(g_{\bar{\beta}}
(\mathcal{O}_L(\bar{\beta},x_i)),+1) + \delta(p)
\end{align*}
with probability at least $1 - p$,
% where $\delta(p) = (p_L + (-\frac{1}{2B} \log p)^{1/2})$,
where $\delta(p) = B \cdot p_L + \frac{\sqrt{\log^2 p-8 B p_l \log p}-\log p}{2}$,
by Chernoff bound, and Lemma~\ref{L:bound}, which assures that an
optimal solution to Problem~\ref{eq:attacker_q} can only over-estimate mistakes.
Moreover,
\begin{align*}
\sum_{i:y_i = +1} &l_{01}(g_{\bar{\beta}}
(\mathcal{O}_L(\bar{\beta},x_i)),+1) \le\\
&\sum_{i:y_i = +1}\sum_{j \in N_i} l(g_{\bar{\beta}}
(\mathcal{O}_L(\bar{\beta},x_i)),+1),
\end{align*}
since $\mathcal{O}_L(\bar{\beta},x_i) \in N_i$ for all $i$ by
construction, and $l$ is an upper bound on $l_{01}$.
Putting everything together, we get the desired result.
\end{proof}

%We empirically evaluate the converging value of $P_A$ empirically as
%shown in Figure~\ref{fig:start}.

\begin{figure}[t]
\centering 
\begin{tabular}{cc}
\includegraphics[scale=0.19]{images/binary_start.png} &
\includegraphics[scale=0.19]{images/continuous_start.png} \\
(a) & (b)
\end{tabular}
\caption{The convergence of $P_A$ based on different number of starting points for (a) Binary, (b) Continuous feature space.}
\label{fig:start}
\end{figure}
Figure~\ref{fig:start} demonstrates that $p_L \rightarrow 0$
quite rapidly for an array of learning algorithms, and for either
discrete or continuous features, as we increase the number of restarts
$L$.
Consequently, in practice retraining with coordinate
greedy nearly minimizes an upper bound on minimal total adversarial
0/1 loss with relatively few restarts of the approximate attacker oracle.

%\begin{algorithm}[thb]
%\caption{Adversarial modification via Coordinate Descent $\mathcal{O}(x,\lambda,\beta)$}
%\label{alg:coordinate}
%\begin{algorithmic}[1]
%\STATE \textbf{Input}: {Malicious instance $x^A, \lambda, \beta$}
% \STATE {Set $k \leftarrow 0$ and let $x^0 \leftarrow x^A$}
% % \WHILE {$k < B$ and $f(x^k) \geq \delta$ }
% \REPEAT 
% % {$|f(x^A)-f(x^k)| \leq \delta$}
% \STATE{Randomly choose index $i_k \in \{1, 2, ..., n\}$ }
% \STATE{$x^{k+1} \leftarrow x^k - \tau_k {[\triangledown Q(x^k)]}_{i_k} e_{i_k}$}
% \STATE {$k \leftarrow k+1$}
% % \UNTIL {$|Q(x^{k})-Q(x^{k-1})| \leq \epsilon$ or $f(x^k) \leq \delta$}
% \UNTIL {$\frac{\ln Q(x^{k})} {\ln Q(x^{k-1})} \leq \epsilon$ or $f(x^k) \leq \delta$}
% % \ENDWHILE
% \STATE {Project $x^{k}$ to the feature space $x' \in X$}
% \STATE \textbf{Output}: {Adversarially optimal instance $x'$.}
%\end{algorithmic}
%\end{algorithm}

%Without loss of generality, we will keep use $\beta$ to denote the parameter set of any learning algorithm for simplicity here.
%Within the algorithm $\tau_k$ is the step size and $e_{i_k}$ is the direction and in our situation, it can be viewed as 1 for each feature dimension. The partial derivation function ${[\triangledown Q(x^k)]}_{i_k}$ corresponds to different learning algorithms and $\lambda$ is the cost sensitive parameter for attacker. 

%To minimize the loss when learning with such adversarial invariances, the learner would apply a retraining strategy to minimize its loss using Algorithm~\ref{algo:retraining}. This retraining process is highly scalable and computationally efficient compared with the constraint generation approach, but may obtain larger loss within an upper bound. 

%We will then discuss the coordinate descent details for different learning models based on different feature spaces. Since the attacker's goal is to minimize $f(x')$ to evade the classifier as well as minimize the modification cost $c(x^A,x')$, the attacker needs to solve the following optimization problem.
%\begin{equation}
%\min \limits_{x'} Q(x') := f(x') +e^{\lambda \sqrt{\sum \limits_{i = 1}^n{ (x^A}_i -{x'}_i)^2 +1}}
%\end{equation}

%Therefore 
%\begin{equation}
%\begin{scriptsize}
%\begin{aligned}
%&{[\triangledown Q(x^k)]}_{i_k} = {[\triangledown f(x^k)]}_{i_k} \\
%- &\exp \left({\lambda \sqrt{\sum \limits_{i = 1}^n{ (x^A}_i -{x'}_i)^2 +1}} \right) \cdot \lambda \frac{{x^A}_i - {x'}_i}{\sqrt{\sum \limits_{i = 1}^n{ (x^A}_i -{x'}_i)^2 +1}} 
%\end{aligned}
%\end{scriptsize}
%\end{equation}

% % svm linear results for enron based on model 2
% \begin{figure}[t]
% \centering 
% \begin{tabular}{cc}
% \includegraphics[scale=0.19]{images/binary2_enron_svm1000.png} &
% \includegraphics[scale=0.19]{images/binary2_enron_svm2000.png} \\
% (a) & (b)
% \end{tabular}
% \caption{SVM linear performance based on different adversarial cost sensitivity $\lambda$ for Enron dataset with different number of binary features as (a) 1000, (b) 2000.}
% \label{fig:ridge_enron}
% \end{figure}

% \section{Continuous Feature Space}
% \label{continuous}



% \begin{algorithm}[thb]
% \caption{Adversarial modification via Coordinate Descent}
% \label{alg:coordinate}
% \begin{algorithmic}[1]
% \STATE \textbf{Input}: {Malicious instance $x^A$}
%  \WHILE{$l \leq Q$}
%  \STATE {Set $k \leftarrow 0$ and let $x^0 \leftarrow x^A$}
%  % \WHILE {$|f(x^A)-f(x^k)| \leq \delta$}
%  \STATE{Randomly choose index $i_k \in \{k_1, k_2, ..., k_m\} = M$ and $|M| \leq B$ }
%  \REPEAT
%  \STATE{$x^{k+1} \leftarrow x^k - \beta_k {[\triangledown f(x^k)]}_{i_k} e_{i_k}$}
%  \STATE {$k \leftarrow k+1$}
%  % \ENDWHILE
%  \UNTIL{$|f(x^{k})-f(x^{k-1})| \leq \epsilon$ or $f(x^k) < \delta$}
%  \STATE {$l \leftarrow l+1$}
%  \ENDWHILE
%  \STATE {Project $x^k$ to the feature space $x' \in X$}
%  \STATE \textbf{Output}: {Adversarially optimal instance $x'$.}
% \end{algorithmic}
% \end{algorithm}

% % (this is for randomly choosing B features to modify, or should we randomly one by one till B?)

% \begin{algorithm}[thb]
% \caption{Adversarial modification via Coordinate Descent}
% \label{alg:coordinate}
% \begin{algorithmic}[1]
% \STATE \textbf{Input}: {Malicious instance $x^A$}
%  \STATE {Set $k \leftarrow 0$ and let $x^0 \leftarrow x^A$}
%  \WHILE {$k < B$ and $f(x^k) \geq \delta$ }
%  \REPEAT 
%  % {$|f(x^A)-f(x^k)| \leq \delta$}
%  \STATE{Randomly choose index $i_k$ }
%  \STATE{$x^{k+1} \leftarrow x^k - \beta_k {[\triangledown f(x^k)]}_{i_k} e_{i_k}$}
%  \STATE {$k \leftarrow k+1$}
%  \UNTIL {$|f(x^{k})-f(x^{k-1})| \leq \epsilon$}
%  \ENDWHILE
%  \STATE {Project $x^{k}$ to the feature space $x' \in X$}
%  \STATE \textbf{Output}: {Adversarially optimal instance $x'$.}
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[thb]
% \caption{Adversarial modification via Coordinate Descent}
% \label{alg:coordinate}
% \begin{algorithmic}[1]
% \STATE \textbf{Input}: {Malicious instance $x^A$}
%  \STATE {Set $k \leftarrow 0$ and let $x^0 \leftarrow x^A$}
%  \WHILE {$d(x^k, x^A) < B$ and $f(x^k) \geq \delta$ }
%  \REPEAT 
%  % {$|f(x^A)-f(x^k)| \leq \delta$}
%  \STATE{Randomly choose index $i_k$ }
%  \STATE{$x^{k+1} \leftarrow x^k - \beta_k {[\triangledown f(x^k)]}_{i_k} e_{i_k}$}
%  \STATE {$k \leftarrow k+1$}
%  \UNTIL {$|f(x^{k})-f(x^{k-1})| \leq \epsilon$}
%  \ENDWHILE
%  \STATE {Project $x^{k}$ to the feature space $x' \in X$}
%  \STATE \textbf{Output}: {Adversarially optimal instance $x'$.}
% \end{algorithmic}
% \end{algorithm}

% Here $d(x_1, x_2) = \sqrt{\sum \limits_{i = 1}^n ({x_1}_i-{x_2}_i)^2}$

% \begin{algorithm}[thb]
% \caption{Adversarial modification via Coordinate Descent}
% \label{alg:coordinate}
% \begin{algorithmic}[1]
% \STATE \textbf{Input}: {Malicious instance $x^A$}
%  \STATE {Set $k \leftarrow 0$ and let $x^0 \leftarrow x^A$}
%  % \WHILE {$k < B$ and $f(x^k) \geq \delta$ }
%  \REPEAT 
%  % {$|f(x^A)-f(x^k)| \leq \delta$}
%  \STATE{Randomly choose index $i_k \in \{1, 2, ..., n\}$ }
%  \STATE{$x^{k+1} \leftarrow x^k - \beta_k {[\triangledown R(x^k)]}_{i_k} e_{i_k}$}
%  \STATE {$k \leftarrow k+1$}
%  \UNTIL {$|R(x^{k})-R(x^{k-1})| \leq \epsilon$ or $f(x^k) \geq \delta$}
%  % \ENDWHILE
%  \STATE {Project $x^{k}$ to the feature space $x' \in X$}
%  \STATE \textbf{Output}: {Adversarially optimal instance $x'$.}
% \end{algorithmic}
% \end{algorithm}

\subsubsection{Continuous Feature Space}
\label{sub:continuous}

For continuous feature space, we assume that both $f(x)$ and
$c(x,\cdot)$ are differentiable in $x$, and propose using the \emph{coordinate descent}
algorithm, which is a special case of coordinate greedy, where the
GreedyImprove step is:
\[
x^{k+1} \leftarrow x^k - \tau_k e_{i_k} \frac{\partial
  Q(x^k)}{\partial x^k_{i_k}},
%{[\triangledown Q(x^k)]}_{i_k}
%e_{i_k},
\]
where $\tau_k$ is the step size and $e_{i_k}$ the direction of $i_k$th
coordinate.
Henceforth, let the origial adversarial instance $x_i$ be given; we
then simplify cost function to be only a function of $x$, denoted $c(x)$.
If the function $f(x)$ is convex and differentiable, our coordinate
descent based algorithm~\ref{alg:coordinate} can always find the
global optima which is the attacker best response $x^*$
\cite{luo1992convergence}, and Proposition~\ref{prop:defender_loss}
applies, by Corollary~\ref{C:convex}.
If $f(x)$ is not convex, then coordinate descent will only converge
to a local optimum.
%However, with random restarts, we can considerably improve solutions
%by choosing the best of several local optima.

%it cannot guarantee that the adversary best response $x^*$ can always
%be found.
% We will discuss these special cases in section~\ref{sub:continuous} and~\ref{sub:discrete}.
%If $f(x)$ is not convex, we will empirically evaluate the 0-1 loss for the defender's loss.

%\begin{equation}
%\begin{scriptsize}
%\begin{aligned}
%&{[\triangledown Q(x^k)]}_{i_k} = {[\triangledown f(x^k)]}_{i_k} \\
%- &\exp \left({\lambda \sqrt{\sum \limits_{i = 1}^n{ (x^A}_i -{x'}_i)^2 +1}} \right) \cdot \lambda \frac{{x^A}_i - {x'}_i}{\sqrt{\sum \limits_{i = 1}^n{ (x^A}_i -{x'}_i)^2 +1}} 
%\end{aligned}
%\end{scriptsize}
%\end{equation}
Now, $\frac{\partial
  Q(x^k)}{\partial x^k_{i_k}} = \frac{\partial
  f(x^k)}{\partial x^k_{i_k}} + \frac{\partial
  c(x^k)}{\partial x^k_{i_k}}$.
Fixing a coordinate $j = i_k$, we derive the partial derivative of
$f(x)$ with respect to coordinate $j$ for several common learning
algorithms, and derive the derivative of $c(x)$ for several natural
cost functions.

%If the feature space is continuous as $X \subseteq R^n$, we need to
%derive ${[\triangledown f(x^k,\beta)]}_{i_k}$ according to different
%learning models.

\paragraph{Kernel SVM}

Consider a general Kernel SVM decision function, for which $f(x) =
\sum_i a_i y_i K(x_i,x)$, where $x_i, y_i$ are the support training data
points, $a_i$ the associated dual SVM parameters, and $K(\cdot,\cdot)$
a kernel function.
Then, $\frac{\partial f(x)}{\partial x_j} = \sum_i a_i y_i
\frac{\partial K(x_i,x)}{\partial x_j}$.
For a linear Kernel, $\frac{\partial K(x_i,x)}{\partial x_j} = x_{ij}$.
For a polynomial Kernal, $\frac{\partial K(x_i,x)}{\partial x_j} = d(c
+ x_i \cdot x)^d x_{ij}$.
For an RBF Kernel, $\frac{\partial K(x_i,x)}{\partial x_j} =
\frac{1}{\sigma^2}K(x_i,x)(x_{ij} - x_j)$.

\paragraph{Logistic Regression}
Given a logistic regression model, for which $f(x) = \frac{1}{1+e^{-\theta^T x}}$, where $\theta$ is the learning parameter. We have $\frac{\partial K(x_i,x)}{\partial x_j} = \frac{\theta_j \cdot e^{-\theta^T x}}{(1+e^{-\theta^T x})^2}$


% \paragraph{Ridge Regression}

% For example, for the Ridge regression $y = {\frac{1}{2} (y-w^Tx)^2 + {||w||}_2}$
% \begin{equation}
% {[\triangledown f(x^k,w)]}_{i_k} = -(y-w^Tx)w_i.
% \end{equation}
% For Bayesian regression $y = x^T A + \epsilon$, where $\epsilon_i \sim N(0,\sigma^2)$,
% \begin{equation}
% {[\triangledown f(x^k,A)]}_{i_k} = A_i.
% \end{equation}
% Note that the estimated coefficient can be derived as $A = {(X^T X)}^{-1} X^T y$.

% For the linear-SVM, $y = \frac{1}{2} w^T w + C \sum \limits_{i = 1}^l \max(1-y_i w^T x_i,0)$,
% \begin{equation}
% {[\triangledown f(x^k,w)]}_{i_k} = C \cdot 
% \begin{cases}
% -y_i w_i ;  &\text{if}\ 1-y_i w^T x_i\ge 0 \\
% 0 ;  &\text{otherwise}
% \end{cases}
% \end{equation}

\paragraph{Neural Network}

For the neural network with sigmoid function as the activation function, if there are three hidden layers,
$g(x) = (1+e^{-h_3(x)})^{-1}$, \\
$h_3(x) = \sum \limits_{t = 1}^{d_3} {w_3}_t {\delta_3}_t (x) +b_3$, \\
${\delta_3}_t (x)= (1+e^{-{h_2}_t(x)})^{-1}$, \\
${h_2}_t(x) = \sum \limits_{j = 1}^{d_2} {w_2}_j {\delta_2}_j (x) +b_2$, \\
${\delta_2}_j (x)= (1+e^{-{h_1}_j(x)})^{-1}$, \\
${h_1}_j(x) = \sum \limits_{p = 1}^{d_1} {w_1}_p {\delta_1}_p (x) +b_1$, \\
${\delta_1}_p (x)= (1+e^{-{h_0}_p(x)})^{-1}$, \\
${h_0}_p(x) = \sum \limits_{l = 1}^{n} {w_1}_l x_l +b_0$, \\

Therefore we have
\begin{equation}
\begin{scriptsize}
\begin{aligned}
&{[\triangledown f(x^k,\beta)]}_{i_k} = g(x)(1-g(x)) \sum \limits_{t = 1}^{d_3} {w_{k_3}}_t {\delta_{k_3}}_t(1-{\delta_{k_3}}_t) \\
&\sum \limits_{j = 1}^{d_2} {w_{k_2}}_j {\delta_{k_2}}_j(1-{\delta_{k_2}}_j) \sum \limits_{p = 1}^{d_1} {w_{k_1}}_p {\delta_{k_1}}_p(1-{\delta_{k_1}}_p) {w_{k_0}}_i.
\end{aligned}
\end{scriptsize}
\end{equation}


For the neural network with rectified linear unit (ReLU) function as the activation function, if there are three hidden layers,
$g(x) = \max(0,h_3(x))$, \\
$h_3(x) = \sum \limits_{t = 1}^{d_3} {w_3}_t {\delta_3}_t (x) +b_3$, \\
${\delta_3}_t (x)= \max(0,{h_2}_t(x))$, \\
${h_2}_t(x) = \sum \limits_{j = 1}^{d_2} {w_2}_j {\delta_2}_j (x) +b_2$, \\
${\delta_2}_j (x)= \max(0,{h_1}_j(x))$, \\
${h_1}_j(x) = \sum \limits_{p = 1}^{d_1} {w_1}_p {\delta_1}_p (x) +b_1$, \\
${\delta_1}_p (x)= \max(0,{h_0}_p(x))$, \\
${h_0}_p(x) = \sum \limits_{l = 1}^{n} {w_1}_l x_l +b_0$, \\

Therefore we have when 
\begin{equation*}
\centering
\begin{scriptsize}
\begin{aligned}
&{[\triangledown f(x^k,\beta)]}_{i_k}  \\
&=
\begin{cases}
 h_3(x) & \sum \limits_{t = 1}^{d_3} {w_3}_t {h_2}_t(x) \sum \limits_{j = 1}^{d_2} {w_2}_j {h_1}_j(x)  \sum \limits_{p = 1}^{d_1} {w_1}_p {h_0}_p(x) {w_{k_0}}_i, \\
 & \text{if}\ {h_3}(x) \cdot \sum \limits_{t = 1}^{d_3} {h_2}_t(x) \cdot \sum \limits_{j = 1}^{d_2} {h_1}_j(x) \cdot \sum \limits_{p = 1}^{d_1} {h_0}_p(x) \ne 0\\
 0, \ &\text{otherwise}.
\end{cases}
\end{aligned}
\end{scriptsize}
\end{equation*}

% % Ridge results for enron
% \begin{figure}[t]
% \centering 
% \begin{tabular}{cc}
% \includegraphics[scale=0.19]{images/ridge_enron1000.png} &
% \includegraphics[scale=0.19]{images/ridge_enron2000.png} \\
% (a) & (b)
% \end{tabular}
% \caption{Ridge regression performance based on different adversarial cost sensitivity $\lambda$ for Enron dataset with different number of features as (a) 100, (b) 2000.}
% \label{fig:ridge_enron}
% \end{figure}

% % Ridge results for mnist

% \begin{figure}[t]
% \centering 
% \begin{tabular}{cc}
% \includegraphics[scale=0.19]{images/ridge_mnist627.png} &
% \includegraphics[scale=0.19]{images/ridge_mnist784.png} \\
% (a) & (b)
% \end{tabular}
% \caption{Ridge regression performance based on different adversarial cost sensitivity $\lambda$ for MNIST dataset with different number of features as (a) 627, (b) 784.}
% \label{fig:ridge_mnist}
% \end{figure}

% \begin{figure}[t]
% \centering 
% \begin{tabular}{cccc}
% \includegraphics[scale=1.00]{images/ridge/0.png} &
% \includegraphics[scale=1.00]{images/ridge/1.png} &
% \includegraphics[scale=1.00]{images/ridge/2.png} &
% \includegraphics[scale=1.00]{images/ridge/3.png} \\
% \includegraphics[scale=1.00]{images/ridge/4.png} &
% \includegraphics[scale=1.00]{images/ridge/5.png} &
% \includegraphics[scale=1.00]{images/ridge/6.png} &
% \includegraphics[scale=1.00]{images/ridge/8.png} \\
% \end{tabular}
% \caption{Modification process of attacker for Ridge regression based by decreasing the cost sensitivity parameter $\lambda$.}
% \label{fig:visual_ridge}
% \end{figure}

% % Bayesian results for enron
% \begin{figure}[t]
% \centering 
% \begin{tabular}{cc}
% \includegraphics[scale=0.19]{images/bayesian_enron1000.png} &
% \includegraphics[scale=0.19]{images/bayesian_enron2000.png} \\
% (a) & (b)
% \end{tabular}
% \caption{Bayesian regression performance based on different adversarial cost sensitivity $\lambda$ for Enron dataset with different number of features as (a) 1000, (b) 2000.}
% \label{fig:bayesian_enron}
% \end{figure}

% % Bayesian results for mnist

% \begin{figure}[t]
% \centering 
% \begin{tabular}{cc}
% \includegraphics[scale=0.19]{images/Bayesian_mnist627.png} &
% \includegraphics[scale=0.19]{images/Bayesian_mnist784.png} \\
% (a) & (b)
% \end{tabular}
% \caption{Bayesian regression performance based on different adversarial cost sensitivity $\lambda$ for MNIST dataset with different number of features as (a) 627, (b) 784.}
% \label{fig:bayesian_mnist}
% \end{figure}

% \begin{figure}[t]
% \centering 
% \begin{tabular}{cccc}
% \includegraphics[scale=1.00]{images/bayesian/0.png} &
% \includegraphics[scale=1.00]{images/bayesian/1.png} &
% \includegraphics[scale=1.00]{images/bayesian/3.png} &
% \includegraphics[scale=1.00]{images/bayesian/5.png} \\
% \includegraphics[scale=1.00]{images/bayesian/6.png} &
% \includegraphics[scale=1.00]{images/bayesian/8.png} &
% \includegraphics[scale=1.00]{images/bayesian/9.png} &
% \includegraphics[scale=1.00]{images/bayesian/10.png} \\
% \end{tabular}
% \caption{Modification process of attacker for Bayesian regression based by decreasing the cost sensitivity parameter $\lambda$.}
% \label{fig:visual_bayesian}
% \end{figure}

% % svm-linear results for enron
% \begin{figure}[t]
% \centering 
% \begin{tabular}{cc}
% \includegraphics[scale=0.19]{images/svm_enron1000.png} &
% \includegraphics[scale=0.19]{images/svm_enron2000.png} \\
% (a) & (b)
% \end{tabular}
% \caption{SVM performance based on different adversarial cost sensitivity $\lambda$ for Enron dataset with different number of features as (a) 1000, (b) 2000.}
% \label{fig:svm_enron}
% \end{figure}

% % svm-linear results for mnist
% % chenge below
% \begin{figure}[t]
% \centering 
% \begin{tabular}{cc}
% \includegraphics[scale=0.19]{images/svm_mnist627.png} &
% \includegraphics[scale=0.19]{images/svm_mnist784.png} \\
% (a) & (b)
% \end{tabular}
% \caption{SVM performance based on different adversarial cost sensitivity $\lambda$ for MNIST dataset with different number of features as (a) 627, (b) 784.}
% \label{fig:svm_mnist}
% \end{figure}

% \begin{figure}[t]
% \centering 
% \begin{tabular}{cccc}
% \includegraphics[scale=1.00]{images/svm/0.png} &
% \includegraphics[scale=1.00]{images/svm/1.png} &
% \includegraphics[scale=1.00]{images/svm/3.png} &
% \includegraphics[scale=1.00]{images/svm/4.png} \\
% \includegraphics[scale=1.00]{images/svm/5.png} &
% \includegraphics[scale=1.00]{images/svm/6.png} &
% \includegraphics[scale=1.00]{images/svm/7.png} &
% \includegraphics[scale=1.00]{images/svm/8.png} \\
% \end{tabular}
% \caption{Modification process of attacker for SVM based by decreasing the cost sensitivity parameter $\lambda$.}
% \label{fig:visual_svm}
% \end{figure}

\subsection{Discrete Feature Space}
\label{sub:discrete}

If the feature space is binary as $X \subseteq \{0,1\}^n$, the attacker would solve the relaxation problem for~\ref{eq:attacker_model} and then project the optimized feature to the binary space.
Therefore, the attacker will apply the similar algorithm Algorithm~\ref{alg:coordinate} and project the feature back to $\{0,1\}$ by thresholding during the 8\emph{th} step in Algorithm~\ref{alg:coordinate}. 

%\begin{proposition}
%\label{prop:defender_loss_discrete}
%The upper bound of defender's loss in adversarial environments is 
%% $L_D \leq \sum \limits_{y_i = -1} l(-w^T x_i) + \sum \limits_{y_i = +1} \max \limits_{{x_i}' \in {x_i}^*} l(w^T {x_i}') + \lambda ||w||_p $.
%${L_D}^A \leq \sum \limits_{x_i \in X \cup R} l_\beta( x_i) + \alpha ||\beta||_p + t \cdot {P}_A$ for binary feature space, where $X$ is the original training set and $R$ represents the total added instances. $t$ denotes the number of malicious instances in $X$ ($t = |X_A|$), and $P_A$ is the probability that the best response $x^*$ would evade the classifier. 
%\end{proposition}
%The proof is similar with that for proposition~\ref{prop:defender_loss_continuous}.
%Figure~\ref{fig:start} shows the converging value of $P_A$ empirically. It is shown that after at most 20 random starts, all different learning models are able to find the best response $x^*$ and Neural Network for both continuous and discrete feature space can even converge with 5 random starts.

% \begin{algorithm}[thbf]
% \caption{Adversarial modification via Coordinate Descent Projection $\mathcal{O}(x,\lambda,\beta)$}
% \label{alg:coordinate}
% \begin{algorithmic}[1]
% \STATE \textbf{Input}: {Malicious instance $x^A, \lambda, \beta$}
%  \STATE {Set $k \leftarrow 0$ and let $x^0 \leftarrow x^A$}
%  % \WHILE {$k < B$ and $f(x^k) \geq \delta$ }
%  \REPEAT 
%  % {$|f(x^A)-f(x^k)| \leq \delta$}
%  \STATE{Randomly choose index $i_k \in \{1, 2, ..., n\}$ }
%  \STATE{$x^{k+1} \leftarrow x^k - \tau_k {[\triangledown Q(x^k)]}_{i_k} e_{i_k}$}
%  \STATE {$k \leftarrow k+1$}
%  % \UNTIL {$|Q(x^{k})-Q(x^{k-1})| \leq \epsilon$ or $f(x^k) \leq \delta$}
%  \UNTIL {$\frac{\ln Q(x^{k})} {\ln Q(x^{k-1})} \leq \epsilon$ or $f(x^k) \leq \delta$}
%  % \ENDWHILE
%  \STATE {Project $x^{k}$ to the binary feature space by thresholding}
%  \STATE \textbf{Output}: {Adversarially optimal instance $x'$.}
% \end{algorithmic}
% \end{algorithm}  


% the lambda results for different models convergence.

